BBRv2+:Towards Balancing Aggressiveness and Fairness with Delay-based Bandwidth Probing

BBRv2, proposed by Google, aims at addressing BBR's shortcomings of unfairness against loss-based congestion control algorithms (CCAs) and excessive retransmissions in shallow-buffered networks. In this paper, we first comprehensively study BBRv2's performance under various network conditions and show that BBRv2 mitigates the shortcomings of BBR. Nevertheless, BBRv2's benefits come with several costs, including the slow responsiveness to bandwidth dynamics as well as the low resilience to random losses. We then propose BBRv2+ to address BBRv2's performance issues without sacrificing its advantages over BBR. To this end, BBRv2+ incorporates delay information into its path model, which cautiously guides the aggressiveness of its bandwidth probing to not reduce its fairness against loss-based CCAs. BBRv2+ also integrates mechanisms for improved resilience to random losses as well as network jitters. Extensive experiments demonstrate the effectiveness of BBRv2+. Especially, it achieves 25% higher throughput and comparable queuing delay in comparison with BBRv2 in high-mobility network scenarios.

==> sections/abandoned.tex <==
\begin{table*}[ht]
    \centering
    \begin{tabularx}{\linewidth}{l|X|c}
        \toprule
        Parameter & Definition & Empirical value \\
        \midrule
         $\mathrm{scale_{comp}}$ & The scale factor of cwnd compensation. & 2 or $\mathrm{{2}/{ln(2)}}$ \\
         $\mathrm{J_{high}}$ & A jitter measurement is considered high if the  $\mathrm{jitter}\geq\mathrm{J_{high}*\mathrm{RTprop}}$. & 0.4 \\
         %$\mathcal{L}_{\mathrm{cruise}}$ & The length (in RTT) of the ProbeCruise state. & random(8, 12) \\
         %$\mathrm{PG_{PT}}$ & The pacing\_gain used in the ProbeTry state. & 1.1 \\
         \multirow{2}{*}{$\mathrm{PU_{th}}$} & $\mathrm{ProbeTry \xrightarrow{} ProbeUp}\ if\ \mathrm{SRTT_{curr\_rtt}}$ $\leq$ $\mathrm{(1+PU_{th})}$ $*$ $\mathrm{SRTT_{prev\_rtt}}$ \newline
         $\mathrm{ProbeUp \xrightarrow{} ProbeUp}\ if\ \mathrm{SRTT_{curr\_rtt}}$ $\leq$ $\mathrm{(1+PU_{th})}$ $*$ $\mathrm{SRTT_{before\_probe}}$  & \multirow{2}{*}{0.02} \\
         %$\mathrm{PA_{th}}$ & $\mathrm{ProbeUp \xrightarrow{} ProbeUp}\ if\ \mathrm{BtlBW_{after\_probe} > PA_{th}*BtlBW_{before\_probe}}$ & 1.2 \\
         
         \multirow{2}{*}{$\mathcal{R}$} &  Expiring the oldest value in the BtlBW max\_filter \textit{if} $\mathcal{R}$ rounds have passed since the last update of BtlBW. & \multirow{2}{*}{25} \\
         
         \multirow{2}{*}{$\mathrm{EBW_{th}}$} &  Expiring the oldest value in the BtlBW max\_filter \textit{if} $\mathrm{MinRTT_{curr\_rtt}}$ $>$ $\mathrm{(1+EBW_{th})}*\mathrm{Min_{4RTT}(RTT)}$ \textit{and} state = ProbeCruise. & \multirow{2}{*}{0.1} \\
         
         \multirow{2}{*}{$\mathrm{MS_{BBRv2}}$} & Mode switching threshold. BBRv2+$\xrightarrow{}$BBRv2 \textit{if} $\mathrm{MinRTT_{curr\_cruise}}$ $>$ $\mathrm{MS_{BBRv2}*RTprop}+\mathrm{MinRTT_{prev\_cruise}}$ \textit{for} two ProbeCruise states.  & \multirow{2}{*}{0.1} \\
         
         \multirow{2}{*}{$\mathrm{MS_{BBRv2+}}$} & Mode switching threshold.
         BBRv2$\xrightarrow{}$BBRv2+ \textit{if}
         $\mathrm{MinRTT_{curr\_cruise}}$ $<$ $\mathrm{MS_{BBRv2+}*RTprop}+\mathrm{RTprop}$
         \textit{for} four ProbeCruise states. & \multirow{2}{*}{0.05} \\
         \bottomrule
    \end{tabularx}
    \caption{The parameters of BBRv2+}
    \label{tab:bbrv2plus_params}
\end{table*}

\begin{figure*}[htbp]
    \begin{minipage}{0.32\linewidth}
        \centering
        \includegraphics[width=1\linewidth]{images/bbr_0.5_0_dynamics}
        \subcaption{BBR}
        \label{fig:bbr_fair_dynamics_shallow}
    \end{minipage}
    \hfill
    \begin{minipage}{0.32\linewidth}
        \centering
        \includegraphics[width=1\linewidth]{images/bbr2_0.5_0_dynamics}
        \subcaption{BBRv2}
        \label{fig:bbr2_fair_dynamics_shallow}
    \end{minipage}
    \hfill
    \begin{minipage}{0.32\linewidth}
        \centering
        \includegraphics[width=1\linewidth]{images/bbr2plus_0.5_0_dynamics}
        \subcaption{BBRv2+}
        \label{fig:bbr2p_fair_dynamics_shallow}
    \end{minipage}
    \caption{Throughput dynamics of BBR/BBRv2/BBRv2+ when Cubic competitors co-exist (0.2xBDP shallow buffer)}
    \label{fig:fair_dynamics_shallow}
\end{figure*}

\begin{figure*}[htbp]
    \begin{minipage}{0.32\linewidth}
        \centering
        \includegraphics[width=1\linewidth]{images/bbr_32_0_dynamics}
        \subcaption{BBR}
        \label{fig:bbr_fair_dynamics_deep}
    \end{minipage}
    \hfill
    \begin{minipage}{0.32\linewidth}
        \centering
        \includegraphics[width=1\linewidth]{images/bbr2_32_0_dynamics}
        \subcaption{BBRv2}
        \label{fig:bbr2_fair_dynamics_deep}
    \end{minipage}
    \hfill
    \begin{minipage}{0.32\linewidth}
        \centering
        \includegraphics[width=1\linewidth]{images/bbr2plus_32_0_dynamics}
        \subcaption{BBRv2+}
        \label{fig:bbr2p_fair_dynamics_deep}
    \end{minipage}
    \caption{Throughput dynamics of BBR/BBRv2/BBRv2+ when Cubic competitors co-exist (32xBDP deep buffer)}
    \label{fig:fair_dynamics_deep}
\end{figure*}
